Merian: A Wide-Field Imaging Survey of Dwarf Galaxies at z~0.06-0.10

We present the Merian Survey, an optical imaging survey optimized for studying the physical properties of bright star-forming dwarf galaxies. Merian is carried out with two medium-band filters ($N708$ and $N540$, centered at $708$ and $540$ nm), custom-built for the Dark Energy Camera (DECam) on the Blanco telescope. Merian covers $\sim 750\,\mathrm{deg}^2$ of equatorial fields, overlapping with the Hyper Suprime-Cam Subaru Strategic Program (HSC-SSP) wide, deep, and ultra-deep fields. When combined with the HSC-SSP imaging data ($grizy$), the new Merian DECam medium-band imaging allows for photometric redshift measurements via the detection of H$\rm\alpha$ and [OIII] line emission flux excess in the $N708$ and $N540$ filters, respectively, at $0.06<z<0.10$. We present an overview of the survey design, observations taken to date, data reduction using the LSST Science Pipelines, including aperture-matched photometry for accurate galaxy colors, and a description of the data included in the first data release (DR1). The key science goals of Merian include: probing the dark matter halos of dwarf galaxies out to their virial radii using high signal-to-noise weak lensing profile measurements, decoupling the effects of baryonic processes from dark matter, and understanding the role of black holes in dwarf galaxy evolution. This rich dataset will also offer unique opportunities for studying extremely metal-poor galaxies via their strong [OIII] emission and H$\rm\alpha$ lines, as well as [OIII] emitters at $z\sim 0.4$, and Ly$\rm\alpha$ emitters at $z\sim 3.3$ and $z\sim 4.8$. Merian showcases the power of utilizing narrow and medium-band filters alongside broad-band filters for sky imaging, demonstrating their synergistic capacity to unveil astrophysical insights across diverse astrophysical phenomena.

==> authors.tex <==
PLEASE ADD YOUR NAME AND ANY ACKNOWLEDGMENTS YOU WOULD LIKE TO BE ADDED TO THE PAPER

Author list (in no particular order)
------------------------------------
Shany Danieli
Erin Kado-Fong
Song Huang
Yifei Luo
Ting Li
Lee S Kelvin
Alexie Leauthaud
Jenny Greene
Xiaojing Lin
Jiaxuan Li
Vivienne Baldassare
Arka Banerjee
Joy Bhattacharyya
Diana Blanco
Alyson Brooks
Zheng Cai
Xinjun Chen
Akaxia Cruz
Robel Geda
Runquan Guan
Sean Johnson
Arun Kannawadi
Stacy Kim
Mingyu Li
Robert Lupton
Charlie Mace
Gustavo E. Medina
Abby Mintz
Yue Pan
Annika Peter
Justin I. Read
Rodrigo Córdova Rosado
Allen Seifert
Erik J. Wasleske
Joseph Wick


Acknowledgment
--------------



\author[0000-0003-0105-9576]{Gustavo E. Medina}
\affiliation{Department of Astronomy \& Astrophysics, University of Toronto, Toronto, ON M5S 3H4, Canada}

